BeyondPixels: A Comprehensive Review of the Evolution of Neural Radiance Fields

Neural rendering combines ideas from classical computer graphics and machine learning to synthesize images from real-world observations. NeRF, short for Neural Radiance Fields, is a recent innovation that uses AI algorithms to create 3D objects from 2D images. By leveraging an interpolation approach, NeRF can produce new 3D reconstructed views of complicated scenes. Rather than directly restoring the whole 3D scene geometry, NeRF generates a volumetric representation called a ``radiance field,'' which is capable of creating color and density for every point within the relevant 3D space. The broad appeal and notoriety of NeRF make it imperative to examine the existing research on the topic comprehensively. While previous surveys on 3D rendering have primarily focused on traditional computer vision-based or deep learning-based approaches, only a handful of them discuss the potential of NeRF. However, such surveys have predominantly focused on NeRF's early contributions and have not explored its full potential. NeRF is a relatively new technique continuously being investigated for its capabilities and limitations. This survey reviews recent advances in NeRF and categorizes them according to their architectural designs, especially in the field of novel view synthesis.

==> subsections/few01.tex <==
\section{Using Zero-One-few Shot}



The multi-mirror catadioptric imaging system allows MirrorNeRF: One-shot Neural Portrait Radiance Field from Multi-mirror Catadioptric Imaging \cite{MirrorNeRF} to reconstruct a 3D scene from a single high-resolution image. MirrorNeRF introduces a novel approach to rendering photo-realistic human portraits for VR/AR applications. The traditional methods for capturing multi-view settings can be expensive and time-consuming. Still, MirrorNeRF provides a low-cost catadioptric imaging system with a single high-resolution camera that enables one-shot portrait reconstruction and rendering. The proposed approach uses a sphere mirror array arranged in a hexagonal pattern and a green screen as a background for foreground segmentation. The target subject is positioned in front of the mirror array for one-shot capture. The system calibrates using red calibration points to obtain the relative pose between the camera and the mirror array. The restored rays sample the plenoptic function of the mirror array, and the system associates image pixels with corresponding 3D points on the mirror surfaces to sample and reconstruct the captured scene. The proposed approach introduces a Neural Warping Radiance Field (NeWRF) to restore the 3D scene and produce photo-realistic images from arbitrary viewpoints. The NeWRF addresses the misalignment caused by manual arrangement and coarse calibration. Additionally, a density regularization scheme is proposed to improve rendering quality and training efficiency by leveraging inherent geometry information in a self-supervised manner. The warping displacement field is conditioned on the mirror to handle the misalignment caused by mirror position deviations. Experimental results demonstrate that the proposed approach is effective and robust in achieving photo-realistic, high-quality, and free-viewpoint rendering of human portraits. However, there are some limitations to the MirrorNeRF system. The requirement that all mirrors be almost on a plane means that the system can only reconstruct the front view of the subject. A high-resolution camera and non-skewed viewing angle are also necessary to achieve high-fidelity results. The training process takes hours for a static scene, but the system's requirements can be reduced to make it portable. However, the system is not suitable for dynamic scenes; incorporating neural priors or techniques to speed up training or making the neural warping field deformable in time series may lead to improvements.


Previous dynamic NeRF methods require dense images as input and can only model a single identity, which limits their applicability. FDNeRF \cite{FDNeRF} requires only a small number of dynamic images and can be used with different people, making it more flexible than existing methods. Using a novel Conditional Feature Warping (CFW) module in the 2D feature space to handle inconsistencies in the dynamic frames and warp them to the desired expression, FDNeRF eliminates the need for dense images and can model different identities with few-shot inputs. The CFW module is conditioned on expression and constrained by 3D geometry and consists of three sub-networks: a ResNet-like feature encoding network, a semantic mapping network, and a conditional warping network. The ResNet-like feature encoding network extracts features from the input frames, and the semantic mapping network maps these features to the target expression. The conditional warping network uses a motion descriptor to guide the warping process, and the aligned feature volumes are obtained through bilinear interpolation sampling. The warping fields are constrained by the 3D geometry represented in the jointly trained NeRF. To reconstruct 3D faces with a desired expression, the Radiance Field Reconstruction method is used. The process first extracts aligned feature vectors from the target feature volumes. Then it feeds them into the reconstruction module to estimate each spatial point's color and density values. The feature vectors, along with the position and direction of the point, are processed by a neural network to produce the final results. The user can set the number of input frames flexibly, and the method eliminates the geometric discrepancy between views by adjusting color-related parameters only in the later stages of the network. To render images, FDNeRF uses a hierarchical sampling strategy and two NeRF networks for coarse and fine reconstructions. The densities estimated by the coarse network are used for important sampling of query points in the fine network, allowing for efficient rendering and high-quality results. However, the authors note that there are limitations to the method, such as inconsistencies in non-face regions and lighting, which can cause blurriness in the result. The authors suggest that future works may overcome these limitations with separate warping fields for different parts and a reflectance field. While there are limitations to the method, the author's suggestions for future works provide a promising direction for further improvements.



==> subsections/fig.tex <==
\begin {figure*}%[!hbtp]
\centering
% \begin{adjustbox}{width=\textwidth}
\begin{tikzpicture}

% draw rectangle node
\node[draw,
    minimum width=2cm,
    minimum height=1cm] at (0,-5) {NeRF};
    
% draw rectangle node
\node[draw,
    minimum width=2cm,
    minimum height=1cm] at (3,-1) {Quality \& Scalability};

% draw rectangle node
\node[draw,
    minimum width=2cm,
    minimum height=1cm] at (3,-5) {Process 1.1};

% draw rectangle node
\node[draw,
    minimum width=2cm,
    minimum height=1cm] at (3,-8) {Process 1.2};

% draw rectangle node
\node[draw,
    minimum width=2cm,
    minimum height=1cm] at (3,-10) {Process 1.3};

\draw[-stealth] (1.02,-5) -- (1.5,-5) -- (1.5,-1) -- (2,-1);
\draw[-stealth] (1.02,-5) -- (1.5,-5) -- (1.5,-5) -- (2,-5);
\draw[-stealth] (1.02,-5) -- (1.5,-5) -- (1.5,-8) -- (2,-8);
\draw[-stealth] (1.02,-5) -- (1.5,-5) -- (1.5,-10) -- (2,-10);

% Change line color
\node[draw=red,
    minimum width=2cm, 
    minimum height=1cm] at (6,0) {Process 2};
    
% Change text color
\node[draw,
    text=red,
    minimum width=2cm, 
    minimum height=1cm] at (6,-2) {Process 4};
    
% Change line color
\node[draw=red,
    minimum width=7cm, 
    minimum height=1cm] at (11.5,0) {Process 3};

% Change text color
\node[draw,
    text=red,
    minimum width=7cm, 
    minimum height=1cm] at (11.5,-2) {Process 5};
 	
\draw[-stealth] (4,-1) -- (4.5, -1) -- (4.5,-0) -- (5,0);
\draw[-stealth] (4,-1) -- (4.5,-1) -- (4.5,-2) -- (5,-2);
\draw[-stealth] (7,0) -- (8,0);
\draw[-stealth] (7,-2) -- (8,-2);

% Change line color
\node[draw=red,
    minimum width=2cm, 
    minimum height=1cm] at (6,-4) {Process 6};

% Change text color
\node[draw,
    text=red,
    minimum width=2cm, 
    minimum height=1cm] at (6,-6) {Process 4};

% Change line color
\node[draw=red,
    minimum width=7cm, 
    minimum height=1cm] at (11.5,-4) {Process 7};
    
% Change text color
\node[draw,
    text=red,
    minimum width=7cm, 
    minimum height=1cm] at (11.5,-6) {Process 9};

\draw[-stealth] (4,-5) -- (4.5,-5) -- (4.5,-4) -- (5,-4);
\draw[-stealth] (4,-5) -- (4.5,-5) -- (4.5,-6) -- (5,-6);
\draw[-stealth] (7,-4) -- (8,-4);
\draw[-stealth] (7,-6) -- (8,-6);



% Change line color
\node[draw,
    text=red,
    minimum width=10cm, 
    minimum height=1cm] at (10,-8) {Process 10};
    
% Change text color
\node[draw,
    text=red,
    minimum width=10cm, 
    minimum height=1cm] at (10,-10) {Process 11};
    
\draw[-stealth] (4,-8) -- (5,-8);
\draw[-stealth] (4,-10) -- (5,-10);

\end{tikzpicture}
% \end{adjustbox}
\caption{A visual representation of the taxonomy of NeRF models categorized based on limitations such as Quality and Scalability, High-Quality Large Dataset, Representing Articulated Objects, and Scene Editing.}
\label{fig:2}
\end{figure*}

==> subsections/intro.tex <==
\section{Introduction}
Neural Radiance Field (NeRF) is a machine learning model that can learn to represent 3D objects in a compact and continuous form, using a neural network. It was introduced in a 2020 research paper by researchers at Google. The model learns to predict the 3D structure of an object from a single 2D image, and can also predict the object's pose, surface properties, and even animation. NeRF has been used in a number of applications, including 3D scene understanding, object tracking, and augmented reality. It's a powerful tool for 3D vision and perception, allowing to creation of 3D models from single 2D images with great accuracy and detail.

"NeRF: Representing Scenes as Neural Radiance Fields for View Synthesis" is the title of the research paper that introduced the Neural Radiance Field (NeRF) model. In the paper, the authors propose a new method for learning a continuous, volumetric representation of a 3D scene from a set of 2D images.
The paper "NeRF: Representing Scenes as Neural Radiance Fields for View Synthesis" introduces the Neural Radiance Field (NeRF) model, a machine learning approach for representing 3D scenes and objects in a continuous and differentiable form using a neural network. The authors show how this representation can be used for various applications such as view synthesis, object tracking, and scene understanding. The paper describes a method of training the NeRF model using a dataset of 3D models and images and demonstrates how the model can be used to generate novel views of a scene or object from an arbitrary viewpoint. The results of the experiments show that NeRF can produce highly detailed and accurate 3D models, and can be used for a range of applications in the field of 3D computer vision and perception.


==> subsections/paper_list.tex <==
Representing Articulated Objects
INeRF: Inverting Neural Radiance Fields for Pose Estimation
Neural Articulated Radiance Field
Animatable Neural Radiance Fields for Modeling Dynamic Human Bodies
HumanNeRF: Free-viewpoint Rendering of Moving People from Monocular Video
BANMo: Building Animatable 3D Neural Models from Many Casual Videos

link
https://arxiv.org/abs/2012.05877
https://arxiv.org/abs/2104.03110
https://zju3dv.github.io/animatable_nerf/
https://grail.cs.washington.edu/projects/humannerf/
https://arxiv.org/abs/2112.12761

GAN
CAMPARI: Camera-Aware Decomposed Generative Neural Radiance Fields
Coordinates Are NOT Lonely -- Codebook Prior Helps Implicit Neural 3D Representations
Pix2NeRF: Unsupervised Conditional p-GAN for Single Image to Neural Radiance Fields Translation
VoxGRAF: Fast 3D-Aware Image Synthesis with Sparse Voxel Grids
HyperNeRFGAN: Hypernetwork approach to 3D NeRF GAN
LOLNeRF: Learn from One Look

link
https://arxiv.org/abs/2103.17269
https://arxiv.org/abs/2210.11170
https://openaccess.thecvf.com/content/CVPR2022/html/Cai_Pix2NeRF_Unsupervised_Conditional_p-GAN_for_Single_Image_to_Neural_Radiance_CVPR_2022_paper.html
https://arxiv.org/abs/2206.07695
https://arxiv.org/abs/2301.11631
https://arxiv.org/abs/2111.09996

Fundamental
Mip-NeRF: A Multiscale Representation for Anti-Aliasing Neural Radiance Fields
Point-NeRF: Point-based Neural Radiance Fields
NeRFusion: Fusing Radiance Fields for Large-Scale Scene Reconstruction
Deforming Radiance Fields with Cages

https://arxiv.org/abs/2103.13415
https://arxiv.org/abs/2201.08845
https://arxiv.org/abs/2203.11283
https://xth430.github.io/deforming-nerf/

scale
FastNeRF: High-Fidelity Neural Rendering at 200FPS
KiloNeRF: Speeding up Neural Radiance Fields with Thousands of Tiny MLPs
Block-NeRF: Scalable Large Scene Neural View Synthesis
Mega-NeRF: Scalable Construction of Large-Scale NeRFs for Virtual Fly-Throughs
DeVRF: Fast Deformable Voxel Radiance Fields for Dynamic Scenes
MobileNeRF: Exploiting the Polygon Rasterization Pipeline for Efficient Neural Field Rendering on Mobile Architectures


https://arxiv.org/abs/2103.10380
https://arxiv.org/abs/2103.13744
https://arxiv.org/abs/2202.05263
https://arxiv.org/abs/2112.10703
https://arxiv.org/abs/2205.15723
https://arxiv.org/abs/2208.00277
